Extreme precipitation forecasting using attention augmented convolutions

Extreme precipitation wreaks havoc throughout the world, causing billions of dollars in damage and uprooting communities, ecosystems, and economies. Accurate extreme precipitation prediction allows more time for preparation and disaster risk management for such extreme events. In this paper, we focus on short-term extreme precipitation forecasting (up to a 12-hour ahead-of-time prediction) from a sequence of sea level pressure and zonal wind anomalies. Although existing machine learning approaches have shown promising results, the associated model and climate uncertainties may reduce their reliability. To address this issue, we propose a self-attention augmented convolution mechanism for extreme precipitation forecasting, systematically combining attention scores with traditional convolutions to enrich feature data and reduce the expected errors of the results. The proposed network architecture is further fused with a highway neural network layer to gain the benefits of unimpeded information flow across several layers. Our experimental results show that the framework outperforms classical convolutional models by 12%. The proposed method increases machine learning as a tool for gaining insights into the physical causes of changing extremes, lowering uncertainty in future forecasts.

==> Makefile <==
# make targets in this Makefile
# ps      PS version of final document
# pdf     PDF version of final document
# dvi     DVI version of final document
# spell   spell check
# count   word & line count
# tar     makes a tar.bz2 of the whole dir
# backup  backs up doc and bib file to ./old


########################################
# change stuff in this block as required
# assume:
#  - name of this dir is $(NAME)
#  - name of the main file is $(NAME)-v$(VERSION), e.g. topo_ad-v0.20

NAME = 		climatenets
DOC = 		$(NAME)
BIB =		$(NAME).bib
WORDS =		$(DOC).tex
GRAPHS = 	
PICTURES =	
DATA =		

########################################

.SUFFIXES:	.tex .fig .dvi .gnp .tif .png .jpg .ps .pdf .spell .dia .eps

LATEX =		latex
PDFLATEX =	pdflatex
BIBTEX = 	bibtex
FIG2DEV =	fig2dev
DIA =		dia
GNUPLOT =	gnuplot
DVIPS = 	dvips -Pwww -t letter
SPELL =		aspell list check -t -d en_GB
PAGER =		less
COMPRESS =	bzip2
COUNT =		wc -l -w
PS2PDF =	ps2pdf
CONVERT =	./convert
JPEG2PS =	jpeg2ps

all:		pdf
dvi:		$(DOC).dvi
ps:		$(DOC).ps
pdf:		$(DOC).pdf
spell:		$(DOC).spell

# This is the generic form - works on Mac, Linux and FreeBSD
# tex -> dvi -> ps -> pdf
.ps.pdf:	$(DOC).ps
		$(PS2PDF) $< $@

# for use on the Mac - direct to pdf rather than tex -> dvi -> ps -> pdf
#.tex.pdf:;	$(PDFLATEX) $<
#		$(BIBTEX) $(<:%.tex=%)
#		$(PDFLATEX) $<
#		$(PDFLATEX) $<


.tex.dvi:;	$(LATEX) $<
		$(BIBTEX) $(<:%.tex=%)
		$(LATEX) $<
		$(LATEX) $<


.fig.eps:;	$(FIG2DEV) -L ps $< $@
		sed 's/F2psDict\ 6400\ dict/F2psDict\ 50\ dict/' $@ > tmp
		mv tmp $@

.tif.eps:;	$(CONVERT) $< $@

.png.eps:;	$(CONVERT) $< $@

.jpg.eps:;	$(JPEG2PS) $< > $@

.dia.eps:;	$(DIA) -e $@ $<

.gnp.eps:;	$(GNUPLOT) $< > $@

.dvi.ps:;	$(DVIPS) -f $* > $@

.tex.spell:;	$(SPELL) < $< > $@
		$(PAGER) $@

$(DOC).dvi:	$(WORDS) $(GRAPHS:%.gnp=%.eps) $(PICTURES:%.fig=%.eps) \
		$(PICTURES:%.dia=%.eps) $(PICTURES:%.png=%.eps) $(PICTURES:%.jpg=%.eps) \
		$(PICTURES:%.tif=%.eps)

count:;		$(COUNT) $(WORDS)

clean:;		rm -rf *.pdf *.dvi *.aux *.log *.ps *.out *.spell *.bbl *.blg \
		*.toc *.lof *.lot *~ *.tar core

# tar
TAR-FILES = 	Makefile $(WORDS) $(BIB) $(GRAPHS) $(PICTURES) $(DATA) \
		$(BACKUP) $(UTIL)

TAR-NAME =	$(DOC).tar
tar:;		@(cd ..; \
		tar -cvf $(NAME)/$(TAR-NAME) $(TAR-FILES:%=$(NAME)/%); \
		$(COMPRESS) $(NAME)/$(TAR-NAME))

# backup
BACKUP-DIR =	$(BACKUP)/$(DOC)
back-up:;	@(mkdir $(BACKUP-DIR); \
		cp -pv $(WORDS) $(BIB) $(GRAPHS) $(DATA) $(PICTURES) \
		$(BACKUP-DIR))

